Foveation-based Mechanisms Alleviate Adversarial Examples

We show that adversarial examples, i.e., the visually imperceptible perturbations that result in Convolutional Neural Networks (CNNs) fail, can be alleviated with a mechanism based on foveations---applying the CNN in different image regions. To see this, first, we report results in ImageNet that lead to a revision of the hypothesis that adversarial perturbations are a consequence of CNNs acting as a linear classifier: CNNs act locally linearly to changes in the image regions with objects recognized by the CNN, and in other regions the CNN may act non-linearly. Then, we corroborate that when the neural responses are linear, applying the foveation mechanism to the adversarial example tends to significantly reduce the effect of the perturbation. This is because, hypothetically, the CNNs for ImageNet are robust to changes of scale and translation of the object produced by the foveation, but this property does not generalize to transformations of the perturbation. As a result, the accuracy after a foveation is almost the same as the accuracy of the CNN without the adversarial perturbation, even if the adversarial perturbation is calculated taking into account a foveation.

==> back_fixations.tex <==
\input{tex/cropclutter}
\section{Fixation-like mechanisms alleviate adversarial examples}
In this section we introduce a hypothesis that shows that fixation mechanism to reduce the effect of adversarial examples. Also we show that the hypothesis is plausible with the  observation made in previous works, that CNNs that are re-trained using adversarial examples do not become robust to them~\citep{gu2014towards,GoodfellowSS_CoRR_2014}.

By a fixation mechanism we mean a transformation of the image that discards a part of the image. After the fixation mechanism, the size of the image in pixels, or the number of neural units, is constrained to be always the same,~\eg a fixation mechanism based on cropping a region resizes the region after the crop, to always take the same image size. This is because the number of neural units in the CNN can not easily change. As a result, the fixation mechanism always produces a transformation of the size and location of the fixated region, in order to mantain  constant the number of input units to the CNN. Another constraint of a fixation mechanism is that it can not invent pixel values to discard the information,~\eg it can not substitute the pixel values of the image by a constant value. For the sake of simplicity, in the following we use a crop of an image region as the fixation mechanism. Note that our definiton is open to more sophisticated mechanisms than a crop, for example, processing different crops of the image at different eccentricites and resolutions, similar to a human visual fixation~\cite{}.
 

Let $T(\Mat{x})$ be the image after the transformation of the fixation mechanism. Due to the linearity hypothesis introduced in the previous section, if the perturbation $\Mat{\epsilon}$ is applied in the same location of the target object, we have that $f(T(\Mat{x}+\Mat{\epsilon}^\star))=\Mat{w}^\prime T(\Mat{x})+\Mat{w}^\prime T(\Mat{\epsilon}^\star)$. The term of the image without perturbation, $\Mat{w}^\prime T(\Mat{x})$, is known to be robust to the change of the scale and location of the target object produced by $T(\Mat{x})$, as CNNs are trained to learn representations that are robust to those transformations. If $T(\Mat{x})$ does not remove any part of the object, applying the transformation $T()$ to the image could even improve the accuracy of the CNN, since $T()$ can removes clutter from the image and the CNN is robust to the canges of scale and translation of the target object.


For the term of the perturbation, $\Mat{w}^\prime T(\Mat{\epsilon}^\star)$, we introduce the hypothesis that the aforementioned robustness of the CNNs to  $T()$  does not generalize to the perturbations. Thus, we argue that the transformation with the fixation mechanism affects perturbation, possibly reducing the alignment between the classifier and the perturbation. Note that CNNs are trained with objects at many different positions and scales, and thus, the representation learns to be robust to the transformations of the object. Yet, objects are visually very different from the perturbations, and hence, the robustness of CNNs to the transformation $T()$ of the objects, might not generalize to the perturbations.


In the following, we provide experimental evidence to support our new hypothesis, and then, we make several predictions from the hypothesis.



\paragraph{Experiments that Support the Hypothesis}
We first compare the accuracy of the adversarial exmaple after and before a fixation mechanism in two different set ups. These two set ups allow to compare a fixation $T()$ that changes the scale or the location of the object by removing clutter, or by removing part of the adversarial perturbation located on the object.


In the first set up, we use the adversarial example used in previous experiments (denoted as \emph{MP}). The fixation mechanism crops the target object using the ground truth bounding box (denoted as \emph{Obj Crop}).  Note that this fixation mechanism guarantees that no parts of the object are removed, and that the clutter is reduced. Also, it produces a change in scale and translation of the image in the location of the object. For the the second set up, we calculate the adversarial example with minimum norm for the image of the cropped target object with the ground truth bounding box (denoted as \emph{MP Obj}).  \emph{MP Obj} are not the same \emph{Crop MP}, since \emph{MP Obj} has the minimum perturbation for the cropped bounding box,~\ie $\Mat{\epsilon}^\star$ is calculated for $T(\Mat{x})$, and \emph{Obj Crop} is $T(\Mat{x}+\Mat{\epsilon}^\star)$ where $\Mat{\epsilon}^\star$ is calculated for $\Mat{x}$. The fixation mechanism that we apply to \emph{MP-Obj} crops a random bounding box of the same size as the object bounding box XXX (denoted as  \emph{Crop MP-Obj}). Later, we provide a control experiment to show that the $10$ crop do not improve in the presence of perturbation over $1$ crop, but they improve in the absence of perturbation. Note that this fixation mechanism introduces clutter to the CNN, but it reduces the amount of perturbation into the CNN since it removes part of the object. Also, note that there is not a change in the scale of the object, only a change of location.


In Fig.~\ref{fig:clutter} we report the accuracy for the aforementioned experiments using different values of the norm of the perturbation before the fixation mechansism. We can see that the accuracy of \emph{MP} and \emph{MP-Obj} are very similar, which indicates that a fixation mechanism does not improves the norm of the minumum adversarial perturbation. Note that this does not contradict our hypothesis: Our hypothesis says that the adversarial example with minumum norm for the image before the transformation, $\Mat{\epsilon}^\star$, will probably not be aligned with the classifier after the transformation, $\Mat{w}^\prime T(\Mat{\epsilon}^\star)$. Yet, this does not mean that there could be another adversarial example for the transformed image, $T(\Mat{x})$, that is aligned with the classifier but not with the image without transformation, $\Mat{x}$, which is the phenomenon that we are observing when we compare  \emph{MP} and \emph{MP-Obj}.


We can see our hypothesis in practice when we observe that \emph{Crop MP} and \emph{Crop MP-Obj} improves the accuracy  of~\emph{MP} and  \emph{MP-Obj} about $40\%$ when the perturbations that are imperceptible, or almost imperceptible! Note that when we increase the value of the norm of the perturbation the accuracy decreases again. This is not surprising, since large perturbations occlude the object by bringing the CNN to work to the non-linear region (Sec~\ref{}). Recall that our hypothesis assumes that the CNN is working in the linear regime, and when we increase the norm of the perturbation this is not the case. We can also observe that the adversarial example slightly improves the accruacy in the absense of adversarial perturbation, due to removing possible distractors in the image. In Table \ref{tbl:clutter} we show the exact value of the accuracy of the results in Fig.~\ref{fig:clutter}, which are about $5\%$ of improvement when there is no perturbation. 


The results with the two different set ups, \emph{Crop MP} and \emph{Crop MP-Obj}, show that the change of location and scale of the object produce big improvements of the accuracy of the adversarial perturbation, independently if they reduce clutter or part of the adversarial perturbation, which is in accordance to our hypothesis. In Table~\ref{tbl:normcomparison}, we show the exact values of the improvements by \emph{Crop MP} and \emph{Crop MP-Obj}. We show how many times the perturbation needs to be increased to produce misclassification when whe use the fixation mechanism. We can see that it is about $5$ time more for \emph{bfgs}, and between $8$ to $w5$ times more for \emph{sign} depending on the CNN and the fixation mechanism. The Table also shows the control experiment that the $10$ crops of \emph{Crop MP-Obj} just produce a small improvement over doing one single crop.



To give a more reassurance about our hypothesis, we evaluate the classification scores for the ground truth object category, after and before the fixation mechanism, for the clean image and the perturbation independently. Thus, we use the property of the linearity of the CNN to compare the term from the clean image,~\ie $f(\Mat{x})-f(T(\Mat{x}) $, and the term from the perturbation,~\ie $\left( f(\Mat{x}+\Mat{\epsilon}^\star)-f(\Mat{x}) \right) - \left( f(T(\Mat{x}+\Mat{\epsilon}^\star))-f(T(\Mat{x}))  \right) $. In Fig.~\cite{fig:XXX}XXX, we show another accumulative histogram as the one in Fig.~\cite{fig:XXX}, that shows the number of images with a change of classification score smaller than the indicated in the horizontal axis. We can see that the term of the perturbation that represents the alignment between the perturbation and the classifier, decreases after $T()$, and the term of the clean object increases.


Finally, we show three different automatic methods to improve the adversarial example with a fixation mechanism that do not use the annotated bounding box. We use the $10$ random crops from the image, which comes already implemented in the Caffe library we use~\cite{Jia_arXiv_2014}. The crops are done on large regions of the image ensuring that the target object is contained in the crops. Then, the classification accuracy is computed by averaging the confidences from the multiple crops. We denote it as \emph{$10$ Crop}. Besides that, we use the state-of-the-art saliency model~\citep{Salicon_2015} to generate $3$ crops from the most salient locations of the image, denoted as \emph{Salcrop} XXX. The saliency map is calcualted with the image with the perturbation, but as shown in ~\citep{Salicon_2015}, the saliency maps can be at at a much lower resolution of the image, and as a result, we find that the accuracy of the saliency map for our application does not degrade with the adversarial perturbation. In order for a fair comparision between \emph{Salcrop} with the \emph{$10$ Crop},  we also report results when using only $3$ random crops from the $10$ crops, called \emph{$3$ Crop}. These methods are applied to the \emph{MP}, and note that in contrast to \emph{Crop MP}, they all can remove part of the location of the object. In Fig.~\ref{fig:clutter} we can see a similar improvement of \emph{MP} by \emph{$10$ Crop}, \emph{$3$ Crop} and \emph{Salcrop}, but the improvement is smaller than for \emph{Crop MP}, probably because the automatic methods may mistakenly remove part of the object, which may degrade the accuracy.
In Table \ref{tbl:clutter} we show the exact value of the accuracy of the results in  Fig.~\ref{fig:clutter}. We envision a fruitful research to design fixation mechanisms to mitigate the adversarial examples.




\paragraph{Comparision to Previous Works to Alleviat Adversarial Examples}
 Previous works that try to alleviate adversarial perturbations are based on training  CNNs that learns to classify the observed adversarial examples~\citep{gu2014towards,GoodfellowSS_CoRR_2014}. Yet, new adversarial examples can be created for the CNN trained with adversarial example, and hence,  a new  re-training of the CNN is needed to take into account the new adversarial examples. Our hypothesis predicts this phenomenon. Since the CNNs are not robust to small transformations of the perturbation, to train the CNN to alleviate the perturbations, the CNN should see the perturbations under many transformations. If we train the CNN with objects under many transformations to be robust to these transformations, it is reasonable to expect that we need to do the same for the transformations.



Finally, observe that if we calculate the adversarial perturbation taking into account which fixation mechanism will be applied to the image, we can find an adversarial perturbation that will misclassify a CNN that uses the fixation mechanism. However, we can apply a second fixation mechanism different from the first one, that will distort the adversarial perturbation in a different way, the new fixation mechanism will alleviate the new adversarial example. This is not possible with the strategy of previous works, since re-training can not applied at test time when the ground truth is not available. 




\begin{table}
	\centering
	\caption{The ratio of perturbation of cropped image and full image, \ie~cropped/full. The samples of the perturbations of cropped and full image need to be both non-zero.}
	\begin{tabular}{ccccccc}
		\toprule
		& \multicolumn{2}{c}{{AlexNet}} & \multicolumn{2}{c}{{GoogLeNet}} & \multicolumn{2}{c}{{VGG}} \\
		\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} ratio & Sign & BFGS & Sign & BFGS & Sign & BFGS \\
		\midrule
		BBOptimal/FullOptimal & 1.5208 & 2.4788 & 2.2713 & 8.8267 & 1.8826 &	5.3728 \\
		BBOptimal/BBCrop & 1.5208 & 1.7027 & 2.2713 & 6.1231 & 1.8826 & 4.0177 \\
		BBCrop/FullOptimal & 6.2484 & 14.4476 & 6.3432 & 25.8569 & 5.0216 & 17.1506 \\
		BBShift/BBOptimal & 4.9085 & 9.1912 & 5.6342 & 19.4249 & 2.9630 & 8.5588 \\
		BBShift1Crop/BBOptimal & 4.5336 & 8.4306 & 5.1256 & 18.1737 & 2.9676 & 8.8038 \\
		\bottomrule
		\label{tbl:normcomparison}
	\end{tabular}
\end{table}




==> summary.tex <==

%\subsection{Summary}
%\label{app:Summary}
%
%We now summarize the two new hypothesis introduced in the paper, and which experiments support them, and the predictions we made from them.
%
%{\bf 1) CNNs act locally linearly on the location of the target object.}
%
%Note that behaving as a linear classifier does not mean that it has been trained as a linear SVM, the induced regularizer by the CNN is quite different than the SVM.
%
%
%
%Supporting experiments:
%\begin{enumerate}
%  \item \emph{Scaling the perturbation}: increasing the norm of the perturbation results in more  misclassification of the images on average~(Fig.~\ref{fig:cross}).
%  \item \emph{Masking the perturbation}: the perturbations localized only on the target object results in a decrease of the accuracy performance that is almost the same as the minimum perturbation for the full image, and the accuracy decreases significantly less when the perturbation is only located on the background (Fig.~\ref{fig:removenoise}). 
%    %\item synthetic noise
%\item \emph{Fig.~$1$ in~\cite{GoodfellowSS_CoRR_2014}:} in this figure from~\cite{GoodfellowSS_CoRR_2014} there is an example in which the minimum \emph{sign} perturbation of an image, $\Mat{\epsilon}$,  is evaluated independently from the image, $\Mat{x}$. The summation of the independently computed classification scores $f(\Mat{x}) + f(\Mat{\epsilon})$, is different from the resulting classification score of $f(\Mat{x}+\Mat{\epsilon})$. From our hypothesis, this is because CNN are locally linear, and the perturbation affects when located on the object. If it is evaluated independently, the object is not present, and thus, it does not produce the same misclassification.
%\item \emph{ReLUs}: ReLUs are applied to the neural responses of the convolutions, and are used in all tested CNNs for ImageNet. They have a linear behavior only if the neural response is active. In this way, if the perturbation is added in a location where the neural responses are active,~\ie the CNN has detected an object, the CNN behaves linearly and the imperceptible perturbation can be propagated through the CNN. Yet, when the neural responses are not active,~\eg in the background where there are no detected objects, any small perturbation would be inhibited by the ReLUs. Thus, the linearity of the CNN is local, and it holds until the perturbation does not occlude the detected object (Fig.~\ref{}). 
%\end{enumerate}
%
%
%The generalization of the cross-network perturbation depends on how similar the CNN models are. In the analyzed CNN networks for ImageNet, are quite different architectures, and the misclassification due to cross-network perturbation is not as harming as it was observed in~\cite{GoodfellowSS_CoRR_2014}, where the networks very very similar with different hyper-parameters. 
% %It is as bad to do cross-network as to do cross-image.
%
%{\bf 2) When the neural responses are in the linear regime (hypothesis 1), CNNs in ImageNet are robust to transformations of scale and location of the target object, but this does not generalize to transformations of the perturbation.}
%
%Supporting experiments:
%\begin{enumerate}
%  \item improvement from change scale (vs clutter)
%  \item improvement from shift (vs 10 shift) -> it removes noise and object, the classifier is robust, but not the perturbation. 10 Crop in original image also improves, and almost does not reduce clutter.
%  \item CNN that are re-trained with adversarial examples in the training set are not robust to new adversarial examples, as reported in~\citep{}. 
%\end{enumerate}
%
%Note that for reproducing these experiments in MNIST dataset, the CNNs have to be robust to shifts and changes of scale, which is not the case of the ones tested in previous works, since they are not trained with data augmentation. 
%
%{\bf Predictions from our hypotheses}
%
%\begin{enumerate}
%\item Applying a fixation mechanism to the adversarial example tends to preserve the component of the neural responses of the target object, and reduce the effect of the component of the perturbation. We have explored 2 a little bit in the paper (Saliency prediction works at a low ressolution-> not susceptible to noise).
%\item Our hypotheses predict that adding adversarial examples to the training set is unfeasible, as we would need a vast quantity of them since the CNN is susceptible to small transformations of the perturbation - but not of the objects. This is plausible with the observation made in the literature~\citep{} that CNNs do not become robust to adversarial examples when the training set is extended by introducing adversarial examples.
%%From our hypothesis,  we would need to extend the dataset with many possible transformations of the perturbations, because CNNs are susceptible to their transformations.
%% Note that this hypothesis also plausible with the observation that CNN that are re-trained with adversarial examples in the training set are not robust to new adversarial examples.
%\end{enumerate}
%
%
%We corroborate our hypothesis by applying changes of scale and location of the object with adversarial perturbation, and we see that even the case of introducing a small shift to the location of the object, that does not change the scale nor remove clutter, bring important improvements of the classification accuracy in the presence of perturbation, which is the first prediction.
%
%From the second prediction, we see two possibilities to alleviate adversarial examples.
%The first one is that CNNs should be robust to transformations of the adversarial perturbations, and trained adding adversarial examples. In this way, it would reduce the sample complexity for learning how to mitigate the adversarial perturbations.
%The second is to use fixation mechanism to exploit the susceptibility of current CNN to distortions of the perturbation.
%
%%For solving the problem by re-training a CNN with adversarial examples, CNNs should be robust to transformations of the adversarial perturbations. In this way, it would reduce the sample complexity for learning how to mitigate the adversarial perturbations. 
%
%% one is to change the CNN to be robust to transformations of the perturbations,  and extend the training set with few adversarial examples, or use fixation mechanism to exploit the susceptibility of current CNN to distortions of the perturbation.
%
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Cross-Image Perturbation}
%\label{app:Figures}
%
%
%
%
%
%%\input{tex/synthetic_example}
%
% 
%We use $3$ different types of perturbations created independently of the image. The first is the random noise that was already use in the previous experiments. The second perturbation is a low frequency version of the random noise  (denoted as \emph{LF} from low frequency). It is the random noise convolved with a low-pass filter which is a patch of $4 \times 4$ pixels with all pixels equal to $1$. Finally, the third perturbation consists on taking the perturbation from one random image, and transferring it to the rest. To do so, we do a copy-and-paste procedure of a patch of $50 \times 50$ XXX pixels randomly selected from the object bounding box in the image that we selected to transfer the perturbation from. This image is always the same, and it has been randomly selected in the dataset. We paste the perturbation 
%
% % \emph{Obj} \emph{Back}
%
% %of the perturbation generated from a different image for each particular network.
%
% 
%% Thus, we select some random pixels inside the regions of the bounding box, and we paste the perturbations generated in another image. In practice, we paste the perturbation of a patch of $? \times ?$ pixels in $50$ pixels of the tested image, and then mask the perturbation with the bounding box. The image from which we crop the perturbation is always the same, and it has been randomly selected in the dataset.
%
%
% 
%%We show examples of the synthetic perturbations in Fig.~\ref{fig:synexamples}. 
%
%
%
%%We compare the synthetic perturbations to the cross-CNN architectures perturbations to validate that the synthetic perturbations are a valid strategy for generating perturbation, see Fig.~\ref{fig:shapes} in the supplementary material. \emph{Synbb} produce similar, or even more, misclassification than cross-CNN architectures perturbations. 
%
%%This is because the cross-CNN architectures perturbations have similar characteristics as the synthetic perturbations, namely the location of the perturbation is on the target object and the texture of the perturbation is similar. 
%
%%[XXX add curves in Fig.~\ref{fig:removenoise} from Fig.~\ref{fig:shapes}]
%%In Fig.~\ref{fig:removenoise}, we can observe that the accuracy of \emph{Lfbb} is lower than \emph{Rbb}, suggesting that low frequency perturbations produce more misclassification on average. 
%
%%Note that  \emph{Lfbb} affects differently when using $L_1$ and $L_{\infty}$ norms.
%
%
%
%%Also, we can see in Fig.~\ref{fig:removenoise}, that \emph{Synbb} and \emph{ISynbb} have a different behavior in harming the accuracy performance.





==> tex/cropclutter.tex <==
\begin{figure*}[t!]
	\centering
	\vspace{-2ex}
	\raisebox{0\height}{\subfloat{\includegraphics[width=0.65\textwidth]{sec4/crop_clutter_legend}}}
	{\renewcommand{\arraystretch}{0.1}
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{ccc}
			\subfloat{\includegraphics[width=.305\textwidth]{sec4/alx_crop_clutter_bfgs_new}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec4/gnt_crop_clutter_bfgs_new}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec4/vgg_crop_clutter_bfgs_new}} 	\vspace{-1ex}\\
		\end{tabular}
	}
	\caption
	{
		\textit{Accuracy of the Foveation Mechanisms.} Accuracy for the three CNNs we evaluate, when varying the $L_1$ norm per pixel of \emph{BFGS}. See Fig.~\ref{fig:clutter2} in ~\ref{app:Results} for results of \emph{Sign} with $L_{\infty}$.}
	\label{fig:clutter}
\end{figure*}


==> tex/fig_energy.tex <==
\begin{figure}[t]
	\centering
	\begin{tikzpicture}
	\matrix[column sep=0.05cm, row sep=0.05cm](layout) {
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/alx_mix_energy_score}}; &
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/gnt_mix_energy_score}}; &
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/vgg_mix_energy_score}}; \\
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/alx_sign_energy_score}}; &
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/gnt_sign_energy_score}}; &
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/vgg_sign_energy_score}}; \\
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/alx_distribution}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/gnt_distribution}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/vgg_distribution}}; \\
	};
	\end{tikzpicture}
	\caption
	{
		\textit{The distribution of the noise energy with respect to classification score.} Quantitative result of mix noise and sign noise where 3 columns are AlexNet, GoogLeNet and VGG from left to right, respectively. First row is accurate classified number with mix noise and sign noise. Second row is L1 energy of mix noise with prediction confidence. Third row is L1 energy of sign noise with prediction confidence. Fourth row classification performance with L1 normalization across models. Fifth row classification performance with L-$\infty$ normalization across models.
	}
	\label{fig:energy}
\end{figure}


==> tex/fig_failedcase.tex <==
\begin{figure}[t]
	\centering
	\begin{tikzpicture}
	\matrix[column sep=0.05cm, row sep=0.05cm](layout) {
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/alx_mix_failedcase}}; &
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/gnt_mix_failedcase}}; &
		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/vgg_mix_failedcase}}; \\
	};
	\end{tikzpicture}
	\caption
	{
		\textit{The statistics on the cases failed to learn out BFGS}. The statistics of the image number failed to BFGS noise with respect to their original prediction score.
	}
	\label{fig:failedcase}
\end{figure}


==> tex/lineareexample18L1.tex <==
\begin{figure*}[t!]
	\centering
	\vspace{-2ex}
	\raisebox{0\height}{\subfloat{\includegraphics[width=0.55\textwidth]{linearity_example/linearexample_legend}}}
	{\renewcommand{\arraystretch}{0.1}
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{ccc}
			\subfloat{\includegraphics[width=.305\textwidth]{linearity_example/alx_bfgs_18}} &
			\subfloat{\includegraphics[width=.305\textwidth]{linearity_example/gnt_bfgs_18}} &
			\subfloat{\includegraphics[width=.305\textwidth]{linearity_example/vgg_bfgs_18}} 	\vspace{-1ex}\\
		\end{tabular}
	}
	\caption
	{
		\textit{Local Linearity of the CNNs.} 
		 Classification score of the ground truth object category for the image in Fig.~\ref{fig:examples}, when varying the $L_1$ norm  per pixel of \emph{BFGS}. See Fig.~\ref{fig:linearexample18},~\ref{fig:linearexample75},~\ref{fig:linearexample174} in~\ref{app:Results} for more examples, and also \emph{Sign} with $L_\infty$ norm.
    }
	\label{fig:linearexample18L1}
\end{figure*}


==> tex/linearitycheck.tex <==
\begin{figure*}[t!]
%	\begin{minipage}{1\textwidth}
	\centering
	\vspace{-2ex}
	\raisebox{0\height}{\subfloat{\includegraphics[width=0.15\textwidth]{sec4/linearity_legend}}}
%	\vspace{-2ex}
	{\renewcommand{\arraystretch}{0.1}%
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{ccc}
			\subfloat{\includegraphics[width=.305\textwidth]{sec4/alx_bfgs_linearity}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec4/gnt_bfgs_linearity}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec4/vgg_bfgs_linearity}} 	\vspace{-1ex}\\
%			\subfloat{\includegraphics[width=.305\textwidth]{sec4/alx_sign_linearity}} &
%			\subfloat{\includegraphics[width=.305\textwidth]{sec4/gnt_sign_linearity}} &
%			\subfloat{\includegraphics[width=.305\textwidth]{sec4/vgg_sign_crop_clutter_bbsal_linf}} \\
		\end{tabular}
	}
%	\vspace{-1ex}
	\caption
	{
		\textit{Linearity Check.}}
	\label{fig:linearity}
\end{figure*}

==> tex/noiseperf.tex <==
%\begin{figure}[t]
%	\centering
%	\begin{tikzpicture}
%	\matrix[column sep=0.05cm, row sep=0.05cm](layout) {
%		\node[inner sep=0pt]	{\includegraphics[width=.05\textwidth]{sec1/classify_num_legend}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/alx_classify_num_prior}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/gnt_classify_num_prior}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/vgg_classify_num_prior}}; \\
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/alx_classify_num}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/gnt_classify_num}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.32\textwidth]{sec1/vgg_classify_num}}; \\
%	};
%	\end{tikzpicture}
%	\caption
%	{
%		\textit{Quantitative results of the effect of magnitude of the noise.} Quantitative result of mix noise and sign noise where 3 columns are AlexNet, GoogleNet and VGG from left to right, respectively. First row is accurate classified number with mix noise and sign noise. Second row is L1 energy of mix noise with prediction confidence. Third row is L1 energy of sign noise with prediction confidence. Fourth row classification performance with L1 normalization across models. Fifth row classification performance with L-$\infty$ normalization across models.
%	}
%	\label{fig:noiseperf}
%\end{figure}
\begin{figure}[t]
	\centering
	{\renewcommand{\arraystretch}{0.1}%
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{lccc}
			%\multicolumn{3}{c}{\includegraphics[width=0.8\textwidth]{fig/legend}} \vspace{-8px}
			%			 \\ 
			%			\raisebox{.35\height}{\subfloat{\includegraphics[width=0.15\textwidth]{fig/legend}}} 
			\raisebox{2.5\height}{\subfloat{\includegraphics[width=.07\textwidth]{sec1/classify_num_legend}}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec1/alx_classify_num_prior}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec1/gnt_classify_num_prior}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec1/vgg_classify_num_prior}} \\
			& 			
			\subfloat{\includegraphics[width=.305\textwidth]{sec1/alx_classify_num}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec1/gnt_classify_num}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec1/vgg_classify_num}} \\
		\end{tabular}
	}
	\vspace{-1ex}
	\caption
	{
		\textit{Quantitative results of the effect of magnitude of the noise.} Quantitative result of mix noise and sign noise where 3 columns are AlexNet, GoogLeNet and VGG from left to right, respectively. First row is accurate classified number with mix noise and sign noise. Second row is L1 energy of mix noise with prediction confidence. Third row is L1 energy of sign noise with prediction confidence. Fourth row classification performance with L1 normalization across models. Fifth row classification performance with L-$\infty$ normalization across models.
	}
	\label{fig:noiseperf}
	\vspace{-2ex}
\end{figure}


==> tex/position.tex <==
%\begin{figure}[t]
%	\centering
%	\begin{tikzpicture}
%	\matrix[column sep=0.05cm, row sep=0.05cm](layout) {
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/alx_mix_position}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/gnt_mix_position}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/vgg_mix_position}}; \\
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/alx_sign_position}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/gnt_sign_position}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/vgg_sign_position}}; \\
%%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/alx_mix_crop_noise}}; &
%%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/gnt_mix_crop_noise}}; &
%%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/vgg_mix_crop_noise}}; \\
%%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/alx_sign_crop_noise}}; &
%%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/gnt_sign_crop_noise}}; &
%%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec2/vgg_sign_crop_noise}}; \\
%	};
%	\end{tikzpicture}
%	\caption
%	{
%		\textit{Quantitative result of evaluation of position of the noise.} Noise distribution analysis where where 3 columns are AlexNet, GoogleNet and VGG from left to right, respectively. First row is analysis of position contribution of mix noise to classification. Second row is analysis of position contribution of sign noise to classification. Third row is classification performance of removing part of mix noise. Forth row is classification performance of removing part of sign noise.
%	}
%	\label{fig:positions}
%\end{figure}

\begin{figure}[b!]
	\centering
	\raisebox{0\height}{\subfloat{\includegraphics[width=0.5\textwidth]{sec2/position_legend}}}
	\vspace{-2ex}
	{\renewcommand{\arraystretch}{0.1}%
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{ccc}
			\subfloat{\includegraphics[width=.305\textwidth]{sec2/alx_mix_position}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec2/gnt_mix_position}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec2/vgg_mix_position}} 	\vspace{-1ex}\\
			\subfloat{\includegraphics[width=.305\textwidth]{sec2/alx_sign_position}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec2/gnt_sign_position}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec2/vgg_sign_position}} \\
		\end{tabular}
	}
%	\vspace{-1ex}
	\caption
	{
		\textit{Accuracy vs. Position of the Perturbation.} Accuracy of AlexNet ($1$st col.), GoogLeNet ($2$nd col.) and VGG ($3$rd col.) networks, changing the proportion of the $L_1$ norm of the perturbation inside the binary mask from the saliency map (\emph{Salmask}), and outside (\emph{Isalmask}) for \emph{bfgs perturbation} ($1$st row) and \emph{sign} ($2$nd row).}
	\label{fig:positions}
%	\vspace{-2ex}
\end{figure}


==> tex/shape.tex <==
%\begin{figure}[t]
%	\centering
%	\begin{tikzpicture}
%	\matrix[column sep=0.05cm, row sep=0.05cm](layout) {
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec3/alx_synthetic_bfgs}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec3/gnt_synthetic_bfgs}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec3/vgg_synthetic_bfgs}}; \\
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec3/alx_synthetic_sign}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec3/gnt_synthetic_sign}}; &
%		\node[inner sep=0pt]	{\includegraphics[width=.33\textwidth]{sec3/vgg_synthetic_sign}}; \\
%	};
%	\end{tikzpicture}
%	\caption
%	{
%		\textit{Classification Performance with the texture factor.} \textit{rsal} is a random map multiplied with the saliency map. \textit{lfsal} is a low-frequency random map multiplied with the saliency map. \textit{syn\_sal} is the synthetic map multiplied with the saliency map. \textit{syn\_bb} is the synthetic map multiplied with the mask generated from bounding box.
%	}
%	\label{fig:shapes}
%\end{figure}

\begin{figure*}[t!]
	\centering
	\vspace{-2ex}
	\raisebox{0\height}{\subfloat{\includegraphics[width=0.6\textwidth]{sec3/synthetic_bb_legend}}}
%	\vspace{-2ex}
	{\renewcommand{\arraystretch}{0.1}%
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{ccc}
			\subfloat{\includegraphics[width=.305\textwidth]{sec3/alx_synthetic_bfgs_new}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec3/gnt_synthetic_bfgs_new}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec3/vgg_synthetic_bfgs_new}} 	\vspace{-1ex}\\
			\subfloat{\includegraphics[width=.305\textwidth]{sec3/alx_synthetic_sign_new}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec3/gnt_synthetic_sign_new}} &
			\subfloat{\includegraphics[width=.305\textwidth]{sec3/vgg_synthetic_sign_new}} \vspace{-1ex}\\
%			\subfloat{\includegraphics[width=.305\textwidth]{sec3/alx_synthetic_bfgs_linf}} &
%			\subfloat{\includegraphics[width=.305\textwidth]{sec3/gnt_synthetic_bfgs_linf}} &
%			\subfloat{\includegraphics[width=.305\textwidth]{sec3/vgg_synthetic_bfgs_linf}} \vspace{-1ex}\\
%			\subfloat{\includegraphics[width=.305\textwidth]{sec3/alx_synthetic_sign_linf}} &
%			\subfloat{\includegraphics[width=.305\textwidth]{sec3/gnt_synthetic_sign_linf}} &
%			\subfloat{\includegraphics[width=.305\textwidth]{sec3/vgg_synthetic_sign_linf}} \\
		\end{tabular}
	}
%	\vspace{-1ex}
	\caption
	{
		\textit{Accuracy \emph{vs.}~Texture of the Perturbation.} 
		Accuracy of the different CNNs, with \emph{bfgs perturbation} ($1$st row), and \emph{sign} ($2$nd row). We change the perturbation norm using $L_1$ norm. We compare the synthetic perturbations: \emph{Rsal}, \emph{Lfsal}, \emph{Synsal} and \emph{Synbb} to the cross-network perturbations, denoted as $X$ $Y$, where $X$ is the network that generated the perturbation - ALX (AlexNet), GNT (GoogLeNet), VGG- and $Y$ indicates the \emph{bfgs perturbation} or \emph{sign}.
%		\textit{Rsal} is a random map multiplied with the saliency map. \textit{Lfsal} is a low-frequency random map multiplied with the saliency map. \textit{syn\_sal} is the synthetic map multiplied with the saliency map. \textit{syn\_bb} is the synthetic map multiplied with the mask generated from bounding box.
	}
	\label{fig:shapes}
%	\vspace{-1ex}
\end{figure*}

